Visual Modality Prompt for Adapting Vision-Language Object Detectors

The zero-shot performance of object detectors degrades when tested on different modalities, such as infrared and depth. While recent work has explored image translation techniques to adapt detectors to new modalities, these methods are limited to a single modality and apply only to traditional detectors. Recently, vision-language detectors, such as YOLO-World and Grounding DINO, have shown promising zero-shot capabilities, however, they have not yet been adapted for other visual modalities. Traditional fine-tuning approaches compromise the zero-shot capabilities of the detectors. The visual prompt strategies commonly used for classification with vision-language models apply the same linear prompt translation to each image, making them less effective. To address these limitations, we propose ModPrompt, a visual prompt strategy to adapt vision-language detectors to new modalities without degrading zero-shot performance. In particular, an encoder-decoder visual prompt strategy is proposed, further enhanced by the integration of inference-friendly modality prompt decoupled residual, facilitating a more robust adaptation. Empirical benchmarking results show our method for modality adaptation on two vision-language detectors, YOLO-World and Grounding DINO, and on challenging infrared (LLVIP, FLIR) and depth (NYUv2) datasets, achieving performance comparable to full fine-tuning while preserving the model's zero-shot capability. Code available at: https://github.com/heitorrapela/ModPrompt.

==> sec/00_abstract.tex <==
\begin{abstract}
 The zero-shot performance of object detectors degrades when tested on different modalities, such as infrared and depth. While recent work has explored image translation techniques to adapt detectors to new modalities, these methods are limited to a single modality and apply only to traditional detectors. Recently, vision-language detectors, such as YOLO-World and Grounding DINO, have shown promising zero-shot capabilities, however, they have not yet been adapted for other visual modalities. Traditional fine-tuning approaches compromise the zero-shot capabilities of the detectors. The visual prompt strategies commonly used for classification with vision-language models apply the same linear prompt translation to each image, making them less effective. To address these limitations, we propose ModPrompt, a visual prompt strategy to adapt vision-language detectors to new modalities without degrading zero-shot performance. In particular, an encoder-decoder visual prompt strategy is proposed, further enhanced by the integration of inference-friendly modality prompt decoupled residual, facilitating a more robust adaptation. Empirical benchmarking results~\footnote{Our code is provided in suppl. materials and will be made public.} show our method for modality adaptation on two vision-language detectors, YOLO-World and Grounding DINO, and on challenging infrared (LLVIP, FLIR) and depth (NYU$_{v2}$) datasets, achieving performance comparable to full fine-tuning while preserving the model's zero-shot capability.
\end{abstract}



















% https://github.com/zhengli97/Awesome-Prompt-Adapter-Learning-for-VLMs
% https://arxiv.org/pdf/2401.17270
% https://arxiv.org/pdf/2211.10277






==> sec/06_backup_material.tex <==
% \begin{table*}[!ht]
%     \centering
%     \resizebox{1.0\textwidth}{!}{%
%     \begin{tabular}{lcccccc}
%         \toprule
%         \multirow{2}{*}[-0.7em]{\textbf{Method}} &  \multicolumn{3}{c}{\textbf{LLVIP - IR}} &  \multicolumn{3}{c}{\textbf{FLIR - IR}} \\
%         \cmidrule(lr){2-4}
%         \cmidrule(lr){5-7}
%         \addlinespace[5pt]        
%         {} & \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{50}$}}} & 
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{75}$}}} &
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP}}} & \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{50}$}}} & 
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{75}$}}} &
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP}}}   \\
%         \midrule
        
        
%         Zero-Shot (ZS)  & 81.00 ± 0.00 & 57.80 ± 0.00 & 53.20 ± 0.00  & 64.70 ± 0.00 & 32.10 ± 0.00 & 34.90 ± 0.00 \\
        

%         \rowcolor[HTML]{EFEFEF}
%         Full Finetuning (FT) & 97.43 ± 0.05 & 77.93 ± 0.21 & 67.73 ± 0.09 & 80.47 ± 1.11 & 41.13 ± 0.41 & 44.17 ± 0.39 \\

%         \midrule

%         Visual Prompt (Fixed) & 70.30 ± 7.89 &	45.67 ± 6.97 &	43.53 ± 5.79  & 45.60 ± 0.08 &	21.90 ± 0.08 &	23.77 ± 0.05 \\
        
%         \rowcolor[HTML]{EFEFEF}
%         Visual Prompt (Random) & 60.13 ± 0.29 &	38.73 ± 0.17 &	36.87 ± 0.12 &  43.27 ± 0.29 &	20.63 ± 0.17 &	22.47 ± 0.12 \\
        
%         Visual Prompt (Padding) & 79.87 ± 1.00 &	51.77 ± 0.90 &	49.30 ± 0.83 &	45.63 ± 1.44 &	22.13 ± 1.08 &	23.87 ± 0.91 \\
        
        
%         \rowcolor[HTML]{EFEFEF}
%         Visual Prompt (WM) & 82.00 ± 1.59 &	53.90 ± 1.06 &	50.90 ± 0.94 & 54.43 ± 0.78 &	26.37 ± 0.54 &	28.67 ± 0.40 \\

%         Visual Prompt (WM$_{v2}$) & 74.10 ± 0.43 & 46.47 ± 0.62 &	44.70 ± 0.22 & 52.43 ± 0.50 &	25.10 ± 0.22 &	27.50 ± 0.22 \\

%         \midrule
%         \rowcolor[HTML]{EFEFEF}
%         \textbf{ModPrompt (Ours)} & \textbf{92.80 ± 0.29} &	\textbf{70.73 ± 1.02} &	\textbf{62.87 ± 0.63} & \textbf{69.03 ± 1.06} &	\textbf{34.87 ± 0.40} &	\textbf{37.33 ± 0.12} \\

        
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Detection performance (AP). YOLO-World-S-v1}
%     \label{tab:main_yolo_world}

% \end{table*}
    
% \begin{table*}[!ht]
%     \centering
%     \resizebox{1.0\textwidth}{!}{%
%     \begin{tabular}{lcccccc}
%         \toprule
%         \multirow{2}{*}[-0.7em]{\textbf{Method}} &  \multicolumn{3}{c}{\textbf{LLVIP - IR}} &  \multicolumn{3}{c}{\textbf{FLIR - IR}} \\
%         \cmidrule(lr){2-4}
%         \cmidrule(lr){5-7}
%         \addlinespace[5pt]        
%         {} & \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{50}$}}} & 
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{75}$}}} &
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP}}} & \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{50}$}}} & 
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{75}$}}} &
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP}}}   \\
%         \midrule
        
%         \rowcolor[HTML]{EFEFEF}
%         Zero-Shot (ZS)  & 85.50 ± 0.00 & 62.70 ± 0.00 & 56.50 ± 0.00  & 64.30 ± 0.00 & 29.30 ± 0.00 & 32.90 ± 0.00 \\
        
%         Head Finetuning (HFT)  & 87.53 ± 0.06 & 65.57 ± 0.23 & 58.10 ± 0.20  & 67.27 ± 0.15 & 33.60 ± 0.26 & 36.20 ± 0.10 \\        

%         \rowcolor[HTML]{EFEFEF}
%         Full Finetuning (FT) & 97.17 ± 0.31 & 79.93 ± 0.83 & 67.83 ± 0.96 & 80.73 ± 0.06 & 42.17 ± 0.78 & 44.17 ± 0.25 \\

%         \midrule

%         Visual Prompt (Fixed) & 83.83 ± 0.06 &	61.53 ± 0.23 &	55.13 ± 0.15  & 64.27 ± 0.06 &	29.47 ± 0.06 &	32.83 ± 0.12 \\
        
%         \rowcolor[HTML]{EFEFEF}
%         Visual Prompt (Random) & 83.87 ± 0.06 &	61.37 ± 0.06 &	55.03 ± 0.06  & 64.03 ± 0.08 &	\textbf{29.50 ± 0.00} &	32.77 ± 0.15 \\
        
%         Visual Prompt (Padding) & 82.73 ± 0.31 &	60.00 ± 0.35 &	55.13 ± 0.15  & 61.73 ± 0.23 &	27.60 ± 0.17 &	31.20 ± 0.20 \\
        
        
%         \rowcolor[HTML]{EFEFEF}
%         Visual Prompt (WM) & 69.57 ± 0.93 &	41.37 ± 1.27 &	40.77 ± 0.87  & 54.73 ± 0.08 &	23.20 ± 0.10 &	27.20 ± 0.10 \\

%         Visual Prompt (WM$_{v2}$) & 69.87 ± 1.12 &	41.77 ± 1.30 &	41.13 ± 0.96  & 54.80 ± 0.10 &	23.13 ± 0.21 &	27.27 ± 0.06 \\

%         \midrule
%         \rowcolor[HTML]{EFEFEF}
%         \textbf{ModPrompt (Ours)} & \textbf{93.13 ± 0.15} &	\textbf{67.17 ± 0.78} &	\textbf{60.10 ± 0.50} & \textbf{65.03 ± 0.05} & 29.23 ± 0.55 & \textbf{32.90 ± 0.26} \\

        
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Detection performance (AP). Grounding Dino Swin T}
%     \label{tab:main_grouding_dino}
% \end{table*}




% \begin{table*}[!h]

% \label{tab:test_tab}
%     \centering
%     \resizebox{0.8\textwidth}{!}{%
%     \begin{tabular}{lccc}
%         \toprule
%         \multirow{2}{*}[-0.7em]{\textbf{Method}} &  \multicolumn{3}{c}{\textbf{FLIR-IR}} \\
%         \cmidrule(lr){2-4}
%         \addlinespace[5pt]        
%         {} & \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{50}$}}} & 
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{75}$}}} &
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP}}}   \\
%         \midrule
        
        
%         Zero-Shot (ZS) &	63.20 ± 0.00 &	32.30 ± 0.00 &	34.20 ± 0.00 \\
        
%         \rowcolor[HTML]{EFEFEF}
%         Text Embeddings &	63.90 ± 0.29 &	31.80 ± 0.08 &	34.53 ± 0.05 \\
    
%         Task Residuals & 63.93 ± 0.29 &	31.77 ± 0.09 &34.53 ± 0.09 \\

%         \midrule
%         \rowcolor[HTML]{EFEFEF}
%         Fixed (30) & 	63.30 ± 0.00 &	32.50 ± 0.00 &	34.30 ± 0.00 \\
%         \rowcolor[HTML]{EFEFEF}
%         Fixed (30)+embeddings	& 63.93 ± 0.26 &	31.80 ± 0.08 &	34.57 ± 0.05 \\
%         \rowcolor[HTML]{EFEFEF}
%         Fixed (30)+task residuals	& 63.93 ± 0.26 &	31.90 ± 0.08 &	34.63 ± 0.05 \\
        
%         Fixed (300)	& 35.50 ± 0.29 &	17.13 ± 0.17 &	18.73 ± 0.09 \\
%         Fixed (300)+embeddings	& 36.20 ± 0.24 &	16.93 ± 0.29 &	19.00 ± 0.16 \\
%         Fixed (300)+task residuals &	36.10 ± 0.16 &	16.90 ± 0.22 &	18.97 ± 0.12 \\


%         \rowcolor[HTML]{EFEFEF}
%         Random (30)	& 62.87 ± 0.39 &	32.17 ± 0.25 &	34.10 ± 0.22 \\
%         \rowcolor[HTML]{EFEFEF}
%         Random (30)+embeddings	& 63.30 ± 0.22 &	31.80 ± 0.16 &	34.30 ± 0.08 \\
%         \rowcolor[HTML]{EFEFEF}
%         Random (30)+task residuals	& 63.30 ± 0.14 &	31.73 ± 0.09 &	34.27 ± 0.12 \\

%         Random (300)	& 28.30 ± 0.29 &	13.60 ± 0.42 &	14.77 ± 0.25 \\
%         Random (300)+embeddings	& 28.67 ± 0.09 & 13.13 ± 0.05 &	14.77 ± 0.05 \\
%         Random (300)+task residuals & 	28.70 ± 0.08 &	13.17 ± 0.05 &	14.77 ± 0.05 \\
        
%         \rowcolor[HTML]{EFEFEF}
%         Padding (30)	& 58.57 ± 0.12 &	29.20 ± 0.08 &	31.33 ± 0.05 \\
%         \rowcolor[HTML]{EFEFEF}        
%         Padding (30)+embeddings	& 59.33 ± 0.05 &	29.03 ± 0.09 &	31.47 ± 0.05 \\
%         \rowcolor[HTML]{EFEFEF}       
%         Padding (30)+task residuals	& 59.23 ± 0.12 &	29.10 ± 0.08 &	31.50 ± 0.08 \\
        
%         Padding (200)	& 23.37 ± 0.12 &	09.63 ± 0.17 &	11.40 ± 0.00 \\
%         Padding (200)+embeddings	& 20.27 ± 0.12 &	08.07 ± 0.05 &	09.67 ± 0.05 \\
%         Padding (200)+task residuals	& 20.30 ± 0.24 &	08.10 ± 0.08 &	09.67 ± 0.05 \\

%         \rowcolor[HTML]{EFEFEF}    
%         WeightMap &	62.77 ± 0.37 &	31.70 ± 0.14 &	33.87 ± 0.17 \\
%         \rowcolor[HTML]{EFEFEF}    
%         WeightMap+embeddings & 63.30 ± 0.16 &	31.43 ± 0.12 &	34.23 ± 0.12 \\
%         \rowcolor[HTML]{EFEFEF}
%         WeightMap+task residuals	& 63.10 ± 0.28 &	31.60 ± 0.29 &	34.20 ± 0.08 \\

        
%         WeightMap+Scale	& 61.90 ± 0.29 &	31.23 ± 0.12 &	33.43 ± 0.12 \\
%         WeightMap+Scale+embeddings	& 62.07 ± 0.31 &	30.60 ± 0.28 &	33.27 ± 0.09 \\
%         WeightMap+Scale+task residuals	& 62.47 ± 0.00 &	30.50 ± 0.00 &	33.50 ± 0.00 \\

%         \midrule
        
%         \rowcolor[HTML]{EFEFEF}
%         ModPrompt+mobilenet& 	71.77 ± 0.41 &	37.17 ± 0.29 &	39.57 ± 0.05 \\
%         \rowcolor[HTML]{EFEFEF}        
%         ModPrompt+mobilenet+embeddings	& 70.83 ± 0.68 &	37.50 ± 0.29 &	39.50 ± 0.22 \\
%         \rowcolor[HTML]{EFEFEF}   
%         ModPrompt+mobilenet+task residuals	& 71.23 ± 0.00 &	37.03 ± 0.00 &	39.43 ± 0.00 \\

        
%         ModPrompt+resnet	& 74.47 ± 0.77 &	38.30 ± 0.43 &	41.10 ± 0.24 \\
%         ModPrompt+resnet+embeddings	& 72.07 ± 0.41 &	37.20 ± 0.37 &	40.03 ± 0.17 \\
%         ModPrompt+resnet+task residuals &	72.73 ± 0.00 &	37.70 ± 0.00 &	40.37 ± 0.00 \\

                
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Detection performance (AP). YOLO-World-S-v2}

% \end{table*}

% \begin{table*}[!h]

% \label{tab:test_tab}
%     \centering
%     \resizebox{0.8\textwidth}{!}{%
%     \begin{tabular}{lccc}
%         \toprule
%         \multirow{2}{*}[-0.7em]{\textbf{Method}} &  \multicolumn{3}{c}{\textbf{NYU$_{v2}$-DEPTH}} \\
%         \cmidrule(lr){2-4}
%         \addlinespace[5pt]        
%         {} & \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{50}$}}} & 
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{75}$}}} &
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP}}}   \\
%         \midrule
        
%         Zero-shot	& 04.80 ± 0.00 &	03.10 ± 0.00 &	03.00 ± 0.00 \\
%         \rowcolor[HTML]{EFEFEF}
%         Fully Fine-Tuning & 49.90 ± 0.08 &	36.40 ± 0.29 &	33.57 ± 0.26 \\
%         \midrule
%         \rowcolor[HTML]{EFEFEF}
%         Fixed (30)	& 04.67 ± 0.05 &	03.07 ± 0.05 &	02.90 ± 0.00 \\
%         \rowcolor[HTML]{EFEFEF}
%         Fixed (300)	& 03.43 ± 0.05 &	02.00 ± 0.08 &	02.10 ± 0.00 \\
%         Random (30)	& 04.23 ± 0.12 &	02.63 ± 0.05 &	02.53 ± 0.05 \\
%         Random (300) &	01.53 ± 0.17 &	00.77 ± 0.12 &	00.87 ± 0.12 \\
%         \rowcolor[HTML]{EFEFEF}
%         Padding (30) &	03.97 ± 0.05 &	02.50 ± 0.00 &	02.43 ± 0.05 \\
%         \rowcolor[HTML]{EFEFEF}
%         Padding (300) &	00.37 ± 0.12 &	00.10 ± 0.08 &	00.17 ± 0.05 \\
%         WeightMap	& 10.67 ± 0.12 &	06.90 ± 0.22 &	06.57 ± 0.05 \\
%         WeightMap+Scale &	10.63 ± 0.12 &	06.67 ± 0.12 &	06.50 ± 0.08 \\
%         \midrule
%         \rowcolor[HTML]{EFEFEF}
%         ModPrompt+mobilenet	& 35.37 ± 0.12 &	25.20 ± 0.24 &	23.27 ± 0.17 \\
%         \rowcolor[HTML]{EFEFEF}
%         ModPrompt+resnet &	\textbf{37.17 ± 0.57} &	\textbf{27.50 ± 0.64} &	\textbf{24.93 ± 0.50} \\
                
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Detection performance (AP). YOLO-World-S-v2}

% \end{table*}


% \begin{table*}[!h]

% \label{tab:test_tab}
%     \centering
%     \resizebox{0.8\textwidth}{!}{%
%     \begin{tabular}{lccc}
%         \toprule
%         \multirow{2}{*}[-0.7em]{\textbf{Method}} &  \multicolumn{3}{c}{\textbf{NYU$_{v2}$-DEPTH}} \\
%         \cmidrule(lr){2-4}
%         \addlinespace[5pt]        
%         {} & \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{50}$}}} & 
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{75}$}}} &
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP}}}   \\
%         \midrule
        
%         Zero-shot	& 08.30 ± 0.00 &	05.60 ± 0.00 &	05.30 ± 0.00 \\
%         \rowcolor[HTML]{EFEFEF}
        
%         TaskRes	& 09.97 ± 0.06 &	06.53 ± 0.06 &	06.20 ± 0.00 \\

%         Fully Fine-Tuning & 51.60 ± 2.09 &	39.17 ± 1.88 &	35.77 ± 1.70 \\
        
%         \midrule
%         \rowcolor[HTML]{EFEFEF}
%         Fixed	& 08.27 ± 0.06 &	05.57 ± 0.06 &	05.27 ± 0.06 \\
%         \rowcolor[HTML]{EFEFEF}
%         Fixed + TR	& 10.00 ± 0.00 &	06.4 ± 0.28 &	06.4 ± 0.28 \\
        
%         Random	& 08.33 ± 0.06 &	05.53 ± 0.06 &	05.27 ± 0.06 \\
%         Random + TR	& 09.90 ± 0.14 &	06.50 ± 0.00 &	06.15 ± 0.07 \\
        
%         \rowcolor[HTML]{EFEFEF}
%         Padding  &	07.63 ± 0.06 &	05.17 ± 0.06 &	04.63 ± 0.06 \\
%         \rowcolor[HTML]{EFEFEF}
%         Padding + TR &	09.27 ± 0.15 &	06.00 ± 0.17 &	05.57 ± 0.15 \\
        
%         WeightMap	& 04.87 ± 0.06 &	02.97 ± 0.06 &	02.97 ± 0.06 \\
%         WeightMap + TR	& 06.17 ± 0.12 &	03.53 ± 0.15 &	03.60 ± 0.10 \\
        
%         \rowcolor[HTML]{EFEFEF}
%         WeightMap+Scale &	05.00 ± 0.10 &	03.07 ± 0.06 &	03.03 ± 0.06 \\
%         \rowcolor[HTML]{EFEFEF}
%         WeightMap+Scale + TR &	06.37 ± 0.12 &	03.63 ± 0.06 &	03.67 ± 0.12 \\
%         \midrule
        
%         ModPrompt+mobilenet	& 21.63 ± 0.32 &	14.60 ± 0.57 &	\textbf{14.17 ± 0.15} \\
%         ModPrompt+mobilenet + TR	& 23.53 ± 1.30 &	15.93 ± 0.45 &	\textbf{15.37 ± 0.65} \\
        
%         \rowcolor[HTML]{EFEFEF}
%         ModPrompt+resnet &	\textbf{21.70 ± 0.20} &	\textbf{15.03 ± 0.29} &	14.13 ± 0.21 \\
%         \rowcolor[HTML]{EFEFEF}
%         ModPrompt+resnet + TR &	\textbf{26.63 ± 0.38} &	\textbf{18.53 ± 0.32} &	17.27 ± 0.46 \\
                
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Detection performance (AP). Grounding Dino}

% \end{table*}




% \begin{table*}[!ht]

%     \centering
%     \resizebox{1.0\textwidth}{!}{%
%     \begin{tabular}{lccqgg}
%         \toprule
%         {\multirow{2}{*}[-0.7em]{\textbf{Detector}}} & \multirow{2}{*}[-0.7em]{\textbf{Method}} & \multirow{2}{*}[-0.7em]{\textbf{Text}} &  \multicolumn{3}{c}{\textbf{NYU$_{v2}$-DEPTH}} \\
%         \cmidrule(lr){4-6}
%         \addlinespace[5pt]        
%         {} & {} & {} & \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{50}$}}} & 
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{75}$}}} &
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP}}}   \\
%         \midrule

%         \rowcolor{white}
%         {} & Zero-Shot (ZS) & - & 04.80 ± 0.00 &    03.10 ± 0.00 &  03.00 ± 0.00 \\
%         {} & Task Residuals & (TR) & 12.37 ± 0.05 &	07.47 ± 0.05 &	07.30 ± 0.00 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{Fixed}} & - &  04.67 ± 0.05 &    03.07 ± 0.05 &  02.90 ± 0.00  \\


%         {} & {}  & TR & 12.47 ± 0.05 &	07.50 ± 0.00 &	07.37 ± 0.05 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         \multirow{4}{*}[0em]{\textbf{YOLO W.}} & \multirow{2}{*}[0em]{\textbf{Random}}   &  - & 04.23 ± 0.12 &    02.63 ± 0.05 &  02.53 ± 0.05 \\
%         {} & {}  & TR & 12.23 ± 0.05 &	07.30 ± 0.08 &	07.20 ± 0.00 \\
        
%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{Padding}}  & - &  03.97 ± 0.05 &  02.50 ± 0.00 &  02.43 ± 0.05  \\


%         {} & {}  & TR & 10.63 ± 0.09 &	05.60 ± 0.08 &	05.97 ± 0.05 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{WeightMap}} & - & 10.67 ± 0.12 &	06.90 ± 0.22 & 06.57 ± 0.05 \\
%         {} & {}  & TR & 13.43 ± 0.09 &	08.07 ± 0.12 &	07.90 ± 0.08 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{ModPrompt}} & - & 37.17 ± 0.57 & 27.50 ± 0.64 & 24.93 ± 0.50  \\
        
%         {} & {} & TR &  \textbf{44.67 ± 0.17} &	\textbf{32.53 ± 0.66} &	\textbf{29.93 ± 0.12} \\

        
%         \midrule
%         \addlinespace[2pt]        
%         \midrule

%             \rowcolor{white}
%         {} & Zero-Shot (ZS) & - & 08.30 ± 0.00 & 05.60 ± 0.00 &  05.30 ± 0.00 \\
        
%         {} &  Task Residuals & (TR) & 09.97 ± 0.06 &    06.53 ± 0.06 &  06.20 ± 0.00 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} &  \multirow{2}{*}[0em]{\textbf{Fixed}}  & - & 08.27 ± 0.06 &    05.57 ± 0.06 &  05.27 ± 0.06 \\
%         {} &  {}     & TR & 10.00 ± 0.00 & 06.40 ± 0.28 &   06.40 ± 0.28 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         \multirow{4}{*}[0em]{\textbf{G. DINO}} &  \multirow{2}{*}[0em]{\textbf{Random}}  &  - & 08.33 ± 0.06 &  05.53 ± 0.06 &  05.27 ± 0.06 \\
%         {} & {}  & TR & 09.90 ± 0.14 &  06.50 ± 0.00 &  06.15 ± 0.07 \\
        
%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} &  \multirow{2}{*}[0em]{\textbf{Padding}}     & - & 07.63 ± 0.06 &  05.17 ± 0.06 &  04.63 ± 0.06 \\
%         {} & {}  & TR & 09.27 ± 0.15 &  06.00 ± 0.17 &  05.57 ± 0.15 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{WeightMap}}  & - & 04.87 ± 0.06 & 02.97 ± 0.06 &  02.97 ± 0.06 \\
%         {} & {}  & TR & 06.17 ± 0.12 &  03.53 ± 0.15 &  03.60 ± 0.10 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{ModPrompt}} & - & 21.70 ± 0.20 & 15.03 ± 0.29 & 14.13 ± 0.21 \\
                
%         {} & {} & TR &  \textbf{26.63 ± 0.38} & \textbf{18.53 ± 0.32} & \textbf{17.27 ± 0.46} \\


%         \bottomrule

        
%     \end{tabular}
%     }
%     \caption{Detection performance (APs) for YOLO-World and Grounding DINO under FLIR-IR and NYU$_{v2}$-Depth. We compared each visual prompt adaptation strategy with or without the learnable task residuals, which are responsible for updating the new task embeddings and not changing the text encoder knowledge.}
%     \label{tab:text_residual_study}
% \end{table*}




% \begin{table}[!ht]

%     \centering
%     \resizebox{1.0\columnwidth}{!}{%
%     \begin{tabular}{lccqgg}
%         \toprule
%         {\multirow{2}{*}[-0.7em]{\textbf{Detector}}} & \multirow{2}{*}[-0.7em]{\textbf{Method}} & \multirow{2}{*}[-0.7em]{\textbf{Text}} &  \multicolumn{3}{c}{\textbf{FLIR-IR}} \\
%         \cmidrule(lr){4-6}
%         \addlinespace[5pt]        
%         {} & {} & {} & \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{50}$}}} & 
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{75}$}}} &
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP}}}   \\
%         \midrule

%         \rowcolor{white}
%         {} & Zero-Shot (ZS) & - &	63.20 ± 0.00 &	32.30 ± 0.00 &	34.20 ± 0.00 \\
        
%         {} &  Task Residuals & (TR) & 63.93 ± 0.29 &	31.77 ± 0.09 &34.53 ± 0.09 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} &  \multirow{2}{*}[0em]{\textbf{Fixed}}  & - & 63.30 ± 0.00 &	32.50 ± 0.00 &	34.30 ± 0.00 \\
%         {} &  {}	 & TR & 63.93 ± 0.26 &	31.90 ± 0.08 &	34.63 ± 0.05 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         \multirow{4}{*}[0em]{\textbf{YOLO W.}} &  \multirow{2}{*}[0em]{\textbf{Random}}	 &  - &  62.87 ± 0.39 &	32.17 ± 0.25 &	34.10 ± 0.22 \\
%         {} & {}	 & TR & 63.30 ± 0.14 &	31.73 ± 0.09 &	34.27 ± 0.12 \\
        
%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} &  \multirow{2}{*}[0em]{\textbf{Padding}}	 & - &  58.57 ± 0.12 &	29.20 ± 0.08 &	31.33 ± 0.05 \\
%         {} & {}	 & TR &  59.23 ± 0.12 &	29.10 ± 0.08 &	31.50 ± 0.08 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{WeightMap}}  & - & 	62.77 ± 0.37 &	31.70 ± 0.14 &	33.87 ± 0.17 \\
%         {} & {}	 & TR &  63.10 ± 0.28 &	31.60 ± 0.29 &	34.20 ± 0.08 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{ModPrompt}} & - &  \textbf{74.47 ± 0.77} & \textbf{38.30 ± 0.43} &	\textbf{41.10 ± 0.24} \\
                
%         {} & {} & TR &  72.73 ± 0.00 &	37.70 ± 0.00 &	40.37 ± 0.00 \\
                 
        
%         \midrule
%         \addlinespace[2pt]        
%         \midrule

    
%         \rowcolor{white}
%         {} & Zero-Shot (ZS) & - &	64.30 ± 0.00 &	29.30 ± 0.00 &	32.90 ± 0.00 \\
%         {} & Task Residuals & (TR) & 65.10 ± 0.18 &	30.20 ± 0.08 & 33.70 ± 0.11 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{Fixed}} & - & 64.27 ± 0.06    & 29.47 ± 0.06  &	32.83 ± 0.12 \\


%         {} & {}	 & TR & 66.53 ± 0.98 &	\textbf{32.83 ± 2.50} &	\textbf{34.83 ± 0.90} \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         \multirow{4}{*}[0em]{\textbf{G. DINO}}  & \multirow{2}{*}[0em]{\textbf{Random}}	 &  - &  64.03 ± 0.08 & 29.50 ± 0.00 & 32.77 ± 0.15 \\
%         {} & {}	 & TR & 66.10 ± 1.08 & 31.40 ± 1.31 & 34.53 ± 0.90 \\
        
%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{Padding}}	 & - &  61.73 ± 0.23 &	27.60 ± 0.17 &	31.20 ± 0.20 \\

              
%         {} & {}	 & TR &  63.33 ± 1.10 &	29.73 ± 1.27 &	32.93 ± 0.90 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{WeightMap}} & - & 	54.73 ± 0.08 & 23.20 ± 0.10 & 27.20 ± 0.10 \\
%         {} & {}	 & TR &  55.60 ± 0.92 &	24.37 ± 0.65 &	28.30 ± 0.66 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{ModPrompt}} & - &  65.03 ± 0.05 & 29.23 ± 0.55 & 32.90 ± 0.26 \\
        
%         {} & {} & TR &  \textbf{67.80 ± 0.14} &	31.10 ± 0.31 &	33.70 ± 0.09 \\


%         \bottomrule

        
%     \end{tabular}
%     }
%     \caption{Detection performance (APs) for YOLO-World and Grounding DINO under FLIR-IR and NYU$_{v2}$-Depth. We compared each visual prompt adaptation strategy with or without the learnable task residuals, which are responsible for updating the new task embeddings and not changing the text encoder knowledge.}
%     \label{tab:text_residual_study}
% \end{table}






% \begin{table}[!ht]

%     \centering
%     \resizebox{1.0\columnwidth}{!}{%
%     \begin{tabular}{lccqgg}
%         \toprule
%         {\multirow{2}{*}[-0.7em]{\textbf{Detector}}} & \multirow{2}{*}[-0.7em]{\textbf{Method}} & \multirow{2}{*}[-0.7em]{\textbf{Text}} &  \multicolumn{3}{c}{\textbf{FLIR-IR}} \\
%         \cmidrule(lr){4-6}
%         \addlinespace[5pt]        
%         {} & {} & {} & \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{50}$}}} & 
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{75}$}}} &
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP}}}   \\
%         \midrule

%         \rowcolor{white}
%         {} & Zero-Shot (ZS) & - &	63.20 ± 0.00 &	32.30 ± 0.00 &	34.20 ± 0.00 \\
        
%         {} &  Task Residuals & (TR) & 63.93 ± 0.29 &	31.77 ± 0.09 &34.53 ± 0.09 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} &  \multirow{2}{*}[0em]{\textbf{Fixed}}  & - & 63.30 ± 0.00 &	32.50 ± 0.00 &	34.30 ± 0.00 \\
%         {} &  {}	 & TR & 63.93 ± 0.26 &	31.90 ± 0.08 &	34.63 ± 0.05 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         \multirow{4}{*}[0em]{\textbf{YOLO W.}} &  \multirow{2}{*}[0em]{\textbf{Random}}	 &  - &  62.87 ± 0.39 &	32.17 ± 0.25 &	34.10 ± 0.22 \\
%         {} & {}	 & TR & 63.30 ± 0.14 &	31.73 ± 0.09 &	34.27 ± 0.12 \\
        
%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} &  \multirow{2}{*}[0em]{\textbf{Padding}}	 & - &  58.57 ± 0.12 &	29.20 ± 0.08 &	31.33 ± 0.05 \\
%         {} & {}	 & TR &  59.23 ± 0.12 &	29.10 ± 0.08 &	31.50 ± 0.08 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{WeightMap}}  & - & 	62.77 ± 0.37 &	31.70 ± 0.14 &	33.87 ± 0.17 \\
%         {} & {}	 & TR &  63.10 ± 0.28 &	31.60 ± 0.29 &	34.20 ± 0.08 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{ModPrompt}} & - &  \textbf{74.47 ± 0.77} & \textbf{38.30 ± 0.43} &	\textbf{41.10 ± 0.24} \\
                
%         {} & {} & TR &  72.73 ± 0.00 &	37.70 ± 0.00 &	40.37 ± 0.00 \\
                 
        
%         \midrule
%         \addlinespace[2pt]        
%         \midrule

    
%         \rowcolor{white}
%         {} & Zero-Shot (ZS) & - &	64.30 ± 0.00 &	29.30 ± 0.00 &	32.90 ± 0.00 \\
%         {} & Task Residuals & (TR) & 65.10 ± 0.18 &	30.20 ± 0.08 & 33.70 ± 0.11 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{Fixed}} & - & 64.27 ± 0.06    & 29.47 ± 0.06  &	32.83 ± 0.12 \\


%         {} & {}	 & TR & 66.53 ± 0.98 &	\textbf{32.83 ± 2.50} &	\textbf{34.83 ± 0.90} \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         \multirow{4}{*}[0em]{\textbf{G. DINO}}  & \multirow{2}{*}[0em]{\textbf{Random}}	 &  - &  64.03 ± 0.08 & 29.50 ± 0.00 & 32.77 ± 0.15 \\
%         {} & {}	 & TR & 66.10 ± 1.08 & 31.40 ± 1.31 & 34.53 ± 0.90 \\
        
%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{Padding}}	 & - &  61.73 ± 0.23 &	27.60 ± 0.17 &	31.20 ± 0.20 \\

              
%         {} & {}	 & TR &  63.33 ± 1.10 &	29.73 ± 1.27 &	32.93 ± 0.90 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{WeightMap}} & - & 	54.73 ± 0.08 & 23.20 ± 0.10 & 27.20 ± 0.10 \\
%         {} & {}	 & TR &  55.60 ± 0.92 &	24.37 ± 0.65 &	28.30 ± 0.66 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{ModPrompt}} & - &  65.03 ± 0.05 & 29.23 ± 0.55 & 32.90 ± 0.26 \\
        
%         {} & {} & TR &  \textbf{67.80 ± 0.14} &	31.10 ± 0.31 &	33.70 ± 0.09 \\

%     \toprule
%         {\multirow{2}{*}[-0.7em]{\textbf{Detector}}} & \multirow{2}{*}[-0.7em]{\textbf{Method}} & \multirow{2}{*}[-0.7em]{\textbf{Text}} &  \multicolumn{3}{c}{\textbf{NYU$_{v2}$-DEPTH}} \\
%         \cmidrule(lr){4-6}
%         \addlinespace[5pt]        
%         {} & {} & {} & \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{50}$}}} & 
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{75}$}}} &
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP}}}   \\
%         \midrule

%         \rowcolor{white}
%         {} & Zero-Shot (ZS) & - & 04.80 ± 0.00 &    03.10 ± 0.00 &  03.00 ± 0.00 \\
%         {} & Task Residuals & (TR) & 12.37 ± 0.05 &	07.47 ± 0.05 &	07.30 ± 0.00 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{Fixed}} & - &  04.67 ± 0.05 &    03.07 ± 0.05 &  02.90 ± 0.00  \\


%         {} & {}  & TR & 12.47 ± 0.05 &	07.50 ± 0.00 &	07.37 ± 0.05 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         \multirow{4}{*}[0em]{\textbf{YOLO W.}} & \multirow{2}{*}[0em]{\textbf{Random}}   &  - & 04.23 ± 0.12 &    02.63 ± 0.05 &  02.53 ± 0.05 \\
%         {} & {}  & TR & 12.23 ± 0.05 &	07.30 ± 0.08 &	07.20 ± 0.00 \\
        
%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{Padding}}  & - &  03.97 ± 0.05 &  02.50 ± 0.00 &  02.43 ± 0.05  \\


%         {} & {}  & TR & 10.63 ± 0.09 &	05.60 ± 0.08 &	05.97 ± 0.05 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{WeightMap}} & - & 10.67 ± 0.12 &	06.90 ± 0.22 & 06.57 ± 0.05 \\
%         {} & {}  & TR & 13.43 ± 0.09 &	08.07 ± 0.12 &	07.90 ± 0.08 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{ModPrompt}} & - & 37.17 ± 0.57 & 27.50 ± 0.64 & 24.93 ± 0.50  \\
        
%         {} & {} & TR &  \textbf{44.67 ± 0.17} &	\textbf{32.53 ± 0.66} &	\textbf{29.93 ± 0.12} \\

        
%         \midrule
%         \addlinespace[2pt]        
%         \midrule

%             \rowcolor{white}
%         {} & Zero-Shot (ZS) & - & 08.30 ± 0.00 & 05.60 ± 0.00 &  05.30 ± 0.00 \\
        
%         {} &  Task Residuals & (TR) & 09.97 ± 0.06 &    06.53 ± 0.06 &  06.20 ± 0.00 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} &  \multirow{2}{*}[0em]{\textbf{Fixed}}  & - & 08.27 ± 0.06 &    05.57 ± 0.06 &  05.27 ± 0.06 \\
%         {} &  {}     & TR & 10.00 ± 0.00 & 06.40 ± 0.28 &   06.40 ± 0.28 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         \multirow{4}{*}[0em]{\textbf{G. DINO}} &  \multirow{2}{*}[0em]{\textbf{Random}}  &  - & 08.33 ± 0.06 &  05.53 ± 0.06 &  05.27 ± 0.06 \\
%         {} & {}  & TR & 09.90 ± 0.14 &  06.50 ± 0.00 &  06.15 ± 0.07 \\
        
%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} &  \multirow{2}{*}[0em]{\textbf{Padding}}     & - & 07.63 ± 0.06 &  05.17 ± 0.06 &  04.63 ± 0.06 \\
%         {} & {}  & TR & 09.27 ± 0.15 &  06.00 ± 0.17 &  05.57 ± 0.15 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{WeightMap}}  & - & 04.87 ± 0.06 & 02.97 ± 0.06 &  02.97 ± 0.06 \\
%         {} & {}  & TR & 06.17 ± 0.12 &  03.53 ± 0.15 &  03.60 ± 0.10 \\

%         \cmidrule(lr){2-6}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{ModPrompt}} & - & 21.70 ± 0.20 & 15.03 ± 0.29 & 14.13 ± 0.21 \\
                
%         {} & {} & TR &  \textbf{26.63 ± 0.38} & \textbf{18.53 ± 0.32} & \textbf{17.27 ± 0.46} \\

%         \bottomrule



%     \end{tabular}
%     }
%     \caption{Detection performance (APs) for YOLO-World and Grounding DINO under FLIR-IR and NYU$_{v2}$-Depth. We compared each visual prompt adaptation strategy with or without the learnable task residuals, which are responsible for updating the new task embeddings and not changing the text encoder knowledge.}
%     \label{tab:text_residual_study}
% \end{table}




% \begin{table*}[!ht]

%     \centering
%     \resizebox{1.0\textwidth}{!}{%
%     \begin{tabular}{lccqggqgg}
%         \toprule
%         {\multirow{2}{*}[-0.7em]{\textbf{Detector}}} & \multirow{2}{*}[-0.7em]{\textbf{Method}} & \multirow{2}{*}[-0.7em]{\textbf{Text}} &  \multicolumn{3}{c}{\textbf{FLIR-IR}} &   \multicolumn{3}{c}{\textbf{NYU$_{v2}$-DEPTH}} \\

%         \cmidrule(lr){4-6}
%         \cmidrule(lr){7-9}
%         \addlinespace[5pt]        
%         {} & {} & {} & \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{50}$}}} & 
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{75}$}}} &
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP}}} & \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{50}$}}} & 
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{75}$}}} &
%         \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP}}}   \\
%         \midrule


%         \rowcolor{white}
%         {} & Zero-Shot (ZS) & - &   63.20 ± 0.00 &  32.30 ± 0.00 &  34.20 ± 0.00 & 04.80 ± 0.00 &    03.10 ± 0.00 &  03.00 ± 0.00 \\
        
%         {} &  Task Residuals & (TR) & 63.93 ± 0.29 &    31.77 ± 0.09 &34.53 ± 0.09  & 12.37 ± 0.05 & 07.47 ± 0.05 &  07.30 ± 0.00 \\

%         \cmidrule(lr){2-9}
%         \rowcolor{white}
%         {} &  \multirow{2}{*}[0em]{\textbf{Fixed}}  & - & 63.30 ± 0.00 &    32.50 ± 0.00 &  34.30 ± 0.00 &  04.67 ± 0.05 &    03.07 ± 0.05 &  02.90 ± 0.00  \\
%         {} &  {}     & TR & 63.93 ± 0.26 &  31.90 ± 0.08 &  34.63 ± 0.05 & 12.47 ± 0.05 &  07.50 ± 0.00 &  07.37 ± 0.05 \\

%         \cmidrule(lr){2-9}
%         \rowcolor{white}
%         \multirow{4}{*}[0em]{\textbf{YOLO-Word.}} &  \multirow{2}{*}[0em]{\textbf{Random}}  &  - &  62.87 ± 0.39 & 32.17 ± 0.25 &  34.10 ± 0.22 & 04.23 ± 0.12 &    02.63 ± 0.05 &  02.53 ± 0.05 \\

%         {} & {}  & TR & 63.30 ± 0.14 &  31.73 ± 0.09 &  34.27 ± 0.12 & 12.23 ± 0.05 &  07.30 ± 0.08 &  07.20 ± 0.00 \\
        
%         \cmidrule(lr){2-9}
%         \rowcolor{white}
%         {} &  \multirow{2}{*}[0em]{\textbf{Padding}}     & - &  58.57 ± 0.12 &  29.20 ± 0.08 &  31.33 ± 0.05 &  03.97 ± 0.05 &  02.50 ± 0.00 &  02.43 ± 0.05  \\
%         {} & {}  & TR &  59.23 ± 0.12 & 29.10 ± 0.08 &  31.50 ± 0.08 & 10.63 ± 0.09 &  05.60 ± 0.08 &  05.97 ± 0.05 \\

%         \cmidrule(lr){2-9}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{WeightMap}}  & - &    62.77 ± 0.37 &  31.70 ± 0.14 &  33.87 ± 0.17 & 10.67 ± 0.12 &  06.90 ± 0.22 & 06.57 ± 0.05 \\
%         {} & {}  & TR &  63.10 ± 0.28 & 31.60 ± 0.29 &  34.20 ± 0.08 & 13.43 ± 0.09 &  08.07 ± 0.12 &  07.90 ± 0.08 \\

%         \cmidrule(lr){2-9}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{ModPrompt}} & - &  \textbf{74.47 ± 0.77} & \textbf{38.30 ± 0.43} &    \textbf{41.10 ± 0.24}  & 37.17 ± 0.57 & 27.50 ± 0.64 & 24.93 ± 0.50  \\
                
%         {} & {} & TR &  72.73 ± 0.00 &  37.70 ± 0.00 &  40.37 ± 0.00 & \textbf{44.67 ± 0.17} & \textbf{32.53 ± 0.66} & \textbf{29.93 ± 0.12} \\
                 
        
%         \midrule
%         \addlinespace[2pt]        
%         \midrule


%         \rowcolor{white}
%         {} & Zero-Shot (ZS) & - &   64.30 ± 0.00 &  29.30 ± 0.00 &  32.90 ± 0.00 & 08.30 ± 0.00 & 05.60 ± 0.00 &  05.30 ± 0.00 \\
%         {} & Task Residuals & (TR) & 65.10 ± 0.18 & 30.20 ± 0.08 & 33.70 ± 0.11 & 09.97 ± 0.06 &    06.53 ± 0.06 &  06.20 ± 0.00 \\

%         \cmidrule(lr){2-9}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{Fixed}} & - & 64.27 ± 0.06    & 29.47 ± 0.06  &   32.83 ± 0.12 & 08.27 ± 0.06 &    05.57 ± 0.06 &  05.27 ± 0.06 \\


%         {} & {}  & TR & 66.53 ± 0.98 &  \textbf{32.83 ± 2.50} & \textbf{34.83 ± 0.90} & 10.00 ± 0.00 & 06.40 ± 0.28 &   06.40 ± 0.28 \\

%         \cmidrule(lr){2-9}
%         \rowcolor{white}
%         \multirow{4}{*}[0em]{\textbf{Grounding DINO}}  & \multirow{2}{*}[0em]{\textbf{Random}}  &  - &  64.03 ± 0.08 & 29.50 ± 0.00 & 32.77 ± 0.15 & 08.33 ± 0.06 &  05.53 ± 0.06 &  05.27 ± 0.06 \\
%         {} & {}  & TR & 66.10 ± 1.08 & 31.40 ± 1.31 & 34.53 ± 0.90 & 09.90 ± 0.14 &  06.50 ± 0.00 &  06.15 ± 0.07 \\
        
%         \cmidrule(lr){2-9}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{Padding}}  & - &  61.73 ± 0.23 &  27.60 ± 0.17 &  31.20 ± 0.20 & 07.63 ± 0.06 &  05.17 ± 0.06 &  04.63 ± 0.06 \\

              
%         {} & {}  & TR &  63.33 ± 1.10 & 29.73 ± 1.27 &  32.93 ± 0.90 & 09.27 ± 0.15 &  06.00 ± 0.17 &  05.57 ± 0.15 \\

%        \cmidrule(lr){2-9}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{WeightMap}} & - &     54.73 ± 0.08 & 23.20 ± 0.10 & 27.20 ± 0.10 & 04.87 ± 0.06 & 02.97 ± 0.06 &  02.97 ± 0.06 \\
%         {} & {}  & TR &  55.60 ± 0.92 & 24.37 ± 0.65 &  28.30 ± 0.66 & 06.17 ± 0.12 &  03.53 ± 0.15 &  03.60 ± 0.10 \\


%         \cmidrule(lr){2-9}
%         \rowcolor{white}
%         {} & \multirow{2}{*}[0em]{\textbf{ModPrompt}} & - &  65.03 ± 0.05 & 29.23 ± 0.55 & 32.90 ± 0.26 & 21.70 ± 0.20 & 15.03 ± 0.29 & 14.13 ± 0.21 \\
        
%         {} & {} & TR &  \textbf{67.80 ± 0.14} & 31.10 ± 0.31 &  33.70 ± 0.09 &  \textbf{26.63 ± 0.38} & \textbf{18.53 ± 0.32} & \textbf{17.27 ± 0.46} \\

%         \bottomrule

%     \end{tabular}
%     }
%     \caption{Detection performance (APs) for YOLO-World and Grounding DINO under FLIR-IR and NYU$_{v2}$-Depth. We compared each visual prompt adaptation strategy with or without the learnable task residuals, which are responsible for updating the new task embeddings and not changing the text encoder knowledge.}
%     \label{tab:text_residual_study}
% \end{table*}








\begin{table}[!ht]
    \centering
    \resizebox{1.0\columnwidth}{!}{%
    \begin{tabular}{lcqgg}
        \toprule
        \multirow{2}{*}[-0.7em]{\textbf{Method}} & \multirow{2}{*}[-0.7em]{\textbf{Variation}} &   \multicolumn{3}{c}{\textbf{LLVIP - IR}} \\
        \cmidrule(lr){3-5}
        \addlinespace[5pt]        
        {} & {} & \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{50}$}}} & 
        \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{75}$}}} &
        \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP}}}   \\
        \midrule


        
        \rowcolor{white}
        \multirow{2}{*}[0em]{\textbf{Fixed}}        & 30     & 61.60 ± 0.75 & 39.93 ± 0.52 & 37.97 ± 0.56 \\
        \cmidrule(lr){2-5}
        {}                                 & 300    & 70.30 ± 7.89 & 45.67 ± 6.97 & 43.53 ± 5.79 \\
        \midrule
        \rowcolor{white}
        \multirow{2}{*}[0em]{\textbf{Random}}       & 30     & 60.13 ± 0.29 & 38.73 ± 0.17 & 36.87 ± 0.12 \\
        \cmidrule(lr){2-5}
        {}                                 & 300    & 56.27 ± 0.46 & 33.73 ± 0.62 & 33.13 ± 0.42 \\
        \midrule
        \rowcolor{white}
        \multirow{2}{*}[0em]{\textbf{Padding}}      & 30     & 79.87 ± 1.00 & 51.77 ± 0.90 & 49.30 ± 0.83 \\
        \cmidrule(lr){2-5}
        {}                                 & 300    & 39.53 ± 2.36 & 15.90 ± 1.02 & 19.07 ± 1.18 \\
        
        \midrule
        \rowcolor{white}
        \multirow{2}{*}[0em]{\textbf{ModPrompt}}    & MB     & \textbf{92.80 ± 0.29} & \textbf{70.73 ± 1.02} & \textbf{62.87 ± 0.63} \\
        \cmidrule(lr){2-5}
        {}                                 & RES    & \textbf{91.03 ± 0.12} & \textbf{68.40 ± 1.10} & \textbf{61.43 ± 0.58} \\
                
        \midrule
        \addlinespace[2pt]        
        \midrule

        % \multirow{2}{*}[-0.7em]{\textbf{Method}} & \multirow{2}{*}[-0.7em]{\textbf{Variation}} &   \multicolumn{3}{c}{\textbf{FLIR - IR}} \\
        % \cmidrule(lr){3-5}
        % \addlinespace[5pt]        
        % {} & {} & \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{50}$}}} & 
        % \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{75}$}}} &
        % \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP}}}   \\
        % \midrule
        % \rowcolor{white}
        % \multirow{2}{*}[0em]{\textbf{Fixed}}        & 30     & 45.60 ± 0.08  & 21.90 ± 0.08 &  23.77 ± 0.05 \\
        % \cmidrule(lr){2-5}
        % {}                                 & 300    & 29.30 ± 0.37  & 13.50 ± 0.54 &  15.00 ± 0.37 \\
        % \midrule
        % \rowcolor{white}
        % \multirow{2}{*}[0em]{\textbf{Random}}       & 30     & 43.27 ± 0.29  & 20.63 ± 0.17 &  22.47 ± 0.12 \\
        % \cmidrule(lr){2-5}
        % {}                                 & 300    & 19.13 ± 0.33  & 09.00 ± 0.42 &  09.80 ± 0.33 \\
        % \midrule
        % \rowcolor{white}
        % \multirow{2}{*}[0em]{\textbf{Padding}}      & 30     & 45.63 ± 1.44  & 22.13 ± 1.08 &  23.87 ± 0.91 \\
        % \cmidrule(lr){2-5}
        % {}                                 & 200    & 00.53 ± 0.12  & 00.17 ± 0.17 &  00.27 ± 0.09 \\
        
        % \midrule
        % \rowcolor{white}
        % \multirow{2}{*}[0em]{\textbf{ModPrompt}}    & MB     & \textbf{66.80 ± 0.29}  & \textbf{35.23 ± 0.38} &  \textbf{36.53 ± 0.12} \\
        % \cmidrule(lr){2-5}
        % {}                                 & RES    & \textbf{69.03 ± 1.06}  & \textbf{34.87 ± 0.40} &  \textbf{37.33 ± 0.12} \\
        
        % \midrule
        % \addlinespace[2pt]        
        % \midrule
        
        \multirow{2}{*}[-0.7em]{\textbf{Method}} & \multirow{2}{*}[-0.7em]{\textbf{Variation}} &   \multicolumn{3}{c}{\textbf{NYU$_{v2}$ - {}Depth}} \\
        \cmidrule(lr){3-5}
        \addlinespace[5pt]        
        {} & {} & \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{50}$}}} & 
        \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP$_{75}$}}} &
        \multicolumn{1}{c}{\multirow{2}{*}[1em]{\textbf{AP}}}   \\
        \midrule
        \rowcolor{white}
        \multirow{2}{*}[0em]{\textbf{Fixed}}        & 30     & 04.67 ± 0.05 &  03.07 ± 0.05 &  02.90 ± 0.00 \\
        \cmidrule(lr){2-5}
        {}                                 & 300    & 03.43 ± 0.05 &  02.00 ± 0.08 &  02.10 ± 0.00 \\
        \midrule
        \rowcolor{white}
        \multirow{2}{*}[0em]{\textbf{Random}}       & 30     & 04.23 ± 0.12 &  02.63 ± 0.05 &  02.53 ± 0.05 \\
        \cmidrule(lr){2-5}
        {}                                 & 300    & 01.53 ± 0.17 &  00.77 ± 0.12 &  00.87 ± 0.12 \\
        \midrule
        \rowcolor{white}
        \multirow{2}{*}[0em]{\textbf{Padding}}      & 30     & 03.97 ± 0.05 &  02.50 ± 0.00 &  02.43 ± 0.05 \\
        \cmidrule(lr){2-5}
        {}                                 & 200    & 00.37 ± 0.12 &  00.10 ± 0.08 &  00.17 ± 0.05 \\
        
        \midrule
        \rowcolor{white}
        \multirow{2}{*}[0em]{\textbf{ModPrompt}}    & MB     & \textbf{35.37 ± 0.12} &  \textbf{25.20 ± 0.24} &  \textbf{23.27 ± 0.17} \\
        \cmidrule(lr){2-5}
        {}                                 & RES    & \textbf{37.17 ± 0.57} &  \textbf{27.50 ± 0.64} &  \textbf{24.93 ± 0.50} \\
        
        
        \bottomrule
    \end{tabular}
    }
    \caption{Detection performance (APs) for YOLO-World under the two main datasets evaluated: LLVIP-IR and NYU$_{v2}$-Depth. We compared the main visual prompt strategies \textit{fixed}, \textit{random}, \textit{padding}, and ModPrompt. The variations consist of the number of prompt pixels (p$_{s}=30$, $200$ or $300$) and for ModPrompt, the MobileNet (MB) or ResNet (RES).}
    \label{tab:ablation_tab}
    \vspace{-.6cm}
\end{table}
